An Equivalence Principle for the Spectrum of Random Inner-Product Kernel Matrices with Polynomial Scalings

We investigate random matrices whose entries are obtained by applying a nonlinear kernel function to pairwise inner products between $n$ independent data vectors, drawn uniformly from the unit sphere in $\mathbb{R}^d$. This study is motivated by applications in machine learning and statistics, where these kernel random matrices and their spectral properties play significant roles. We establish the weak limit of the empirical spectral distribution of these matrices in a polynomial scaling regime, where $d, n \to \infty$ such that $n / d^\ell \to \kappa$, for some fixed $\ell \in \mathbb{N}$ and $\kappa \in (0, \infty)$. Our findings generalize an earlier result by Cheng and Singer, who examined the same model in the linear scaling regime (with $\ell = 1$). Our work reveals an equivalence principle: the spectrum of the random kernel matrix is asymptotically equivalent to that of a simpler matrix model, constructed as a linear combination of a (shifted) Wishart matrix and an independent matrix sampled from the Gaussian orthogonal ensemble. The aspect ratio of the Wishart matrix and the coefficients of the linear combination are determined by $\ell$ and the expansion of the kernel function in the orthogonal Hermite polynomial basis. Consequently, the limiting spectrum of the random kernel matrix can be characterized as the free additive convolution between a Marchenko-Pastur law and a semicircle law. We also extend our results to cases with data vectors sampled from isotropic Gaussian distributions instead of spherical distributions.

==> general_nonlinear_old.tex <==
\subsection{General Nonlinear Kernels}
\label{sec:general_f}

In this section, we extend the equivalence principle presented in Theorem~\ref{thm:equivalence} to the case when the kernel $f_d$ in \eref{A_f} is a general function beyond polynomials. Our analysis uses the following comparison inequality.

\begin{lemma}\label{lemma:s1s2}
Let $A$ be the matrix in \eref{A_f}, and $\hat A$ be another matrix constructed in the same way, but with $f_d$ replaced by $\hat f_d$. For $z \in C_+$ with $\eta = \im[z]$, let $s(z)$ and $\hat{s}(z)$ denote the Stieltjes transforms of $A$ and $\hat A$, respectively. Then we have
\[
\abs{s(z) - \hat s(z)} \le \frac{1}{\eta^2} \big(\EE_{\xi \sim \taumeasure} [f_d(\xi) - \hat f_d(\xi)]^2\big)^{1/2} + \mathcal{O}_\prec\Big(\frac{1}{\eta\sqrt{n}}\Big).
\]
\end{lemma}
\begin{proof}
By the triangular inequality,
\begin{align}
\abs{s(z) - \hat s(z)} &\le \abs{\EE s(z) - \EE \hat s(z)} + \abs{s(z) - \EE s(z)} + \abs{\hat s(z) - \EE \hat s(z)}\\
&\le \EE \abs{s(z) - \hat s(z)} + \mathcal{O}_\prec((\eta \sqrt n)^{-1}),
\end{align}
where the second step uses the standard concentration inequality collected in Lemma~\ref{lemma:sz_concentration}. To complete the proof, we apply the perturbation estimate \eref{s_diff} in Lemma~\ref{lemma:sG_perturbation} and H\"{o}lder's inequality to write
\[
\EE \abs{s(z) - \hat s(z)} \le \frac{1}{\sqrt{n} \eta^2} \EE \norms{A - \hat A}_\mathrm{F} \le \frac{1}{\sqrt{n} \eta^2} (\EE \norms{A - \hat A}_\mathrm{F}^2)^{1/2} \le \frac{1}{\eta^2} \big(\EE [f_d(\xi) - \hat f_d(\xi)]^2\big)^{1/2}.
\]
In the last step, we have used the fact that, for any $i, j \in [n]$ with $i \neq j$, the probability distribution of $\sqrt{n} (A_{ij} - \hat A_{ij})$ equals to that of $f_d(\xi) - \hat f_d(\xi)$, with $\xi \sim \taumeasure$.
\end{proof}

In what follows, we establish an equivalence principle for the matrix in \eref{A_f} under the following assumption on the function $f_d$.
\begin{assumption}\label{assumption:f}
Let $\xi^{(d)} \sim \taumeasure$. The function $f_d$ in \eref{A_f} satisfies the following conditions:
\begin{enumerate}
\item[(a)] For each $k \in \N_0$, we have
\begin{equation}\label{eq:cok_limit}
\EE [f_d(\xi^{(d)}) q_k^{(d)}(\xi^{(d)})] \xrightarrow{d\to\infty} \co_k,
\end{equation}
for some finite numbers $\set{\co_k}$.

\item[(b)] $\sigma^2 \bydef \sum_{k = 0}^\infty \co_k^2 < \infty$, and $\EE [f_d(\xi^{(d)})]^2 \to \sigma^2$ as $d \to \infty$.
\end{enumerate}
\end{assumption}

In the above expressions, we have temporarily reintroduced the superscripts in $\xi^{(d)}$ and $q_k^{(d)}$ to emphasize that both depend on the dimension $d$. As in the rest of the paper, we will omit the superscripts and make the $d$-dependence implicit in subsequent discussions.

%It is possible to further relax the conditions in Assumption~\ref{assumption:f} and consider a larger class of functions that can be  approximated by a finite number of Gegenbauer polynomials uniformly over $d$. See \cite[Sec. 3.2]{cheng2013SpectrumRandom} for details. On the other hand, 

\begin{remark}\label{rem:assumption_sufficient}
When $f_d = f$ is a function that does not depend on $d$, there are simple sufficient conditions one can use to verify that Assumption~\ref{assumption:f} is satisfied. Specifically, by \cite[Lemma C.2, Lemma C.5]{cheng2013SpectrumRandom} (see also Lemma~\ref{lemma:f_cond} in Appendix~\ref{appendix:ortho_poly}), a function $f$ satisfies Assumption~\ref{assumption:f} if (a) $f$ is locally bounded, \emph{i.e.}, $\sup_{\,\abs{x} \le t} \abs{f(x)} < \infty$ for every $t > 0$; and (b) $\EE [f^2(z) \charfn(\,\abs{z} \ge t)] \to 0$ as $t \to \infty$, where $z \sim \mathcal{N}(0, 1)$. Moreover, in this case the limits in Assumption~\ref{assumption:f} can be explicitly computed as
\begin{equation}\label{eq:co_Hermite}
\co_k = \EE [f(z) h_k(z)] \quad\text{and}\quad \sigma^2 = \sum_{k=0}^\infty \co_k^2 = \EE f^2(z),
\end{equation}
where $h_k(x)$ is the $k$th (normalized) Hermite polynomial (see Appendix~\ref{appendix:ortho_poly}).
\end{remark}
\begin{theorem}\label{thm:equivalence_f}
Let $A$ be the matrix in \eref{A_f} with the function $f_d$ satisfying the conditions in Assumption~\ref{assumption:f}. $s_A(z)$ denotes its Stieltjes transform. Fix $\ratio, \tau > 0$, and suppose that $n/d^\ell = \ratio  + \mathcal{O}(d^{-1/2})$, and $z = E + i\eta$ with $\abs{E} \le \tau^{-1}$ and $\tau \le \eta \le \tau^{-1}$. Then, $s_{\mA}(z) \to m(z)$ almost surely as $d \to \infty$, where $m(z)$ is the unique solution in $C_+$ to the equation
\begin{equation}\label{eq:m_equation_f}
m(z)\Big(z + \frac{\coa m(z)}{1 + \cob m(z)} + \coch m(z)\Big) + 1 = 0.
\end{equation}
Here, $\coa = \co_\ell^2$, $\cob = \co_\ell \sqrt{\ell!\ratio}$, $\coch = \sigma^2 - \sum_{0 \le k \le \ell} \co_k^2$, and $\set{\co_k}, \sigma^2$ are the constants defined in Assumption~\ref{assumption:f}.
\end{theorem}
\begin{remark}
Recall from \sref{heuristics} that the self-consistent equation \eref{m_equation_f} characterizes the free additive convolution of a (shifted) MP law and the semicircle law. It follows that the statement of Theorem~\ref{thm:equivalence_f} can still be interpreted in terms of an equivalence principle: the limiting ESD of $A$ is equivalent to that of 
\[
B = \co_\ell B_\ell + (\sigma^2 - \textstyle\sum_{0 \le k \le \ell} \co_k^2)^{1/2} H
\]
where $B_\ell$ is the matrix defined in \eref{Bell} and $H$ is a GOE matrix independent of $B_\ell$.
\end{remark}
\begin{proof}
By Assumption~\ref{assumption:f}(b), for any fixed (small) $c > 0$, there exists some integer $L \ge \ell+1$ such that
\begin{equation}\label{eq:co_conv}
\sigma^2 - (\eta^4 c^2/24) \le \textstyle\sum_{0 \le k \le L - 1} \co_k^2 \le \sigma^2.
\end{equation}
For $\xi \sim \taumeasure$, we write $\inprod{f, g} \bydef \EE[f(\xi) g(\xi)]$ and $\norm{f} \bydef [\EE f^2(\xi)]^{1/2}$. Now define two functions
\[
P_{f_{d}, L}(x) = f_d(x) - \textstyle\sum_{0 \le k \le L} \inprod{f_d, q_k} q_k(x)
\]
and
\[
\hat f_d(x) = \textstyle\sum_{0 \le k \le L-1} \co_k q_k(x) + \hat \co_{L} q_{L}(x),
\]
where $\hat \co_{L} \bydef (\sigma^2 - \sum_{0 \le k \le L-1} \co_k^2)^{1/2}$. We then have
\begin{align}
\norms{f_d - \hat f_d}^2 &= \norms{\textstyle\sum_{0 \le k \le L-1} (\inprod{f_d, q_k} - \co_k) q_k(x) + (\inprod{f_d, q_L} - \hat \co_L) q_L(x) + P_{f_{d}, L}(x)}^2\\
&= \textstyle\sum_{0 \le k \le L-1} (\inprod{f_d, q_k} - \co_k)^2 + (\inprod{f_d, q_L} - \hat \co_L)^2 + (\,\norm{f_d}^2 - \sum_{0 \le k \le L} \inprod{f_d, q_k}^2)\\
&\le (\co_L - \hat \co_L)^2 + (\sigma^2 - \textstyle\sum_{0 \le k \le L} \co_k^2) + \eta^4 c^2/24, \qquad \text{for all sufficiently large } d.\label{eq:fhf_0}
\end{align}
In the second step, we have used the property that the Gengenbauer polynomials are orthonormal [see \eref{ortho_poly}] In the last step, we have used Assumption~\ref{assumption:f}(a), which guarantees that the inequality \eref{fhf_0} holds for all $d \ge d(L, c)$, where $d(L, c)$ is some integer that might depend on $L$ and $c$. By \eref{co_conv}, $\hat \co_L^2 \le \eta^4 c^2/24$ and $\co_L^2 \le \eta^4 c^2/24$. We can then further bound the right-hand side of \eref{fhf_0} as
\begin{equation}\label{eq:f_approx}
\norms{f_d - \hat f_d}^2 \le 2 \co_L^2 + 2 \hat \co_L^2 + (\sigma^2 - \textstyle\sum_{0 \le k \le L} \co_k^2) + \eta^4 c^2/24 \le \eta^4 c^2/4,
\end{equation}
for all sufficiently large $d$.

Let $\widehat A$ be a matrix constructed according to \eref{A_f} but with the function $f_d$ replaced by $\hat f_d$. Let $s_{\widehat A}$ be its Stieltjes transform. By construction, $\hat f_d$ is a linear combination of $L+1$ Gegenbauer polynomials. Thus, we can apply Theorem~\ref{thm:equivalence} to get
\begin{equation}\label{eq:sfm}
\abs{s_{\widehat A}(z) - m(z)} \prec \frac{1}{\sqrt{d}},
\end{equation}
where $m(z) \in \C_+$ is the solution to \eref{m_equation_f}. By using the triangular inequality in the first step, and by applying Lemma~\ref{lemma:s1s2} and \eref{sfm} in the second step, we have
\begin{align}
\abs{s_A(z) - m(z)} &\le \abs{s_A(z) - s_{\widehat A}(z)} + \abs{s_{\widehat A}(z) - m(z)}\\
&\le \frac{1}{\eta^2} [\EE (f_d(\xi) - \hat f_d(\xi)^2]^{1/2} + \mathcal{O}_\prec\Big(\frac{1}{\eta\sqrt{n}}\Big) +  \mathcal{O}_\prec\Big(\frac{1}{\sqrt{d}}\Big)\\
&\le c/2 +  \mathcal{O}_\prec\Big(\frac{1}{\sqrt{d}}\Big),
\end{align}
where the last inequality follows from \eref{f_approx}. Thus, for any $D > 0$,
\[
\P(\,\abs{s_A(z) - m(z)} > c) < d^{-D}
\]
for all sufficiently large $d$. Applying the Borel-Cantelli lemma (for any fixed $D > 1$), we can then conclude that $s_A(z)$ converges to $m(z)$ almost surely.
\end{proof}

